From discrete particles to continuum fields near a boundary

An expression for the stress tensor near an external boundary of a discrete mechanical system is derived explicitly in terms of the constituents' degrees of freedom and interaction forces. Starting point is the exact and general coarse graining formulation presented by Goldhirsch in [I. Goldhirsch, Gran. Mat., 12(3):239-252, 2010], which is consistent with the continuum equations everywhere but does not account for boundaries. Our extension accounts for the boundary interaction forces in a self-consistent way and thus allows the construction of continuous stress fields that obey the macroscopic conservation laws even within one coarse-graining width of the boundary. The resolution and shape of the coarse-graining function used in the formulation can be chosen freely, such that both microscopic and macroscopic effects can be studied. The method does not require temporal averaging and thus can be used to investigate time-dependent flows as well as static and steady situations. Finally, the fore-mentioned continuous field can be used to define 'fuzzy' (highly rough) boundaries. Two discrete particle method simulations are presented in which the novel boundary treatment is exemplified, including a chute flow over a base with roughness greater than a particle diameter.

==> Figures/2D.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s02}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$x$\end{tabular}}%
\psfrag{s03}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$z$\end{tabular}}%
\psfrag{s05}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s06}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s07}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{100}%
\psfrag{x02}[t][t]{200}%
\psfrag{x03}[t][t]{300}%
\psfrag{x04}[t][t]{400}%
\psfrag{x05}[t][t]{500}%
\psfrag{x06}[t][t]{600}%
%
% yticklabels:
\psfrag{v01}[r][r]{100}%
\psfrag{v02}[r][r]{200}%
\psfrag{v03}[r][r]{300}%
%
% Figure:
\resizebox{6.4cm}{!}{\includegraphics{2D.matlab.eps}}%
\end{psfrags}%
%
% End 2D.matlab.tex


==> Figures/2DStressZZ.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s02}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$x$\end{tabular}}%
\psfrag{s03}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$z$\end{tabular}}%
\psfrag{s05}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$|\V{\sigma}|_2$\end{tabular}}%
\psfrag{s06}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s07}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{0}%
\psfrag{x02}[t][t]{1}%
\psfrag{x03}[t][t]{2}%
\psfrag{x04}[t][t]{3}%
\psfrag{x05}[t][t]{4}%
\psfrag{x06}[t][t]{5}%
%
% yticklabels:
\psfrag{v01}[l][l]{0}%
\psfrag{v02}[l][l]{0.5}%
\psfrag{v03}[l][l]{1}%
\psfrag{v04}[l][l]{1.5}%
\psfrag{v05}[l][l]{2}%
\psfrag{v06}[l][l]{2.5}%
\psfrag{v07}[l][l]{3}%
\psfrag{v08}[r][r]{-0.5}%
\psfrag{v09}[r][r]{0}%
\psfrag{v10}[r][r]{0.5}%
\psfrag{v11}[r][r]{1}%
\psfrag{v12}[r][r]{1.5}%
\psfrag{v13}[r][r]{2}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{2DStressZZ.matlab.eps}}%
\end{psfrags}%
%
% End 2DStressZZ.matlab.tex


==> Figures/2DTractionZ.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s02}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$x$\end{tabular}}%
\psfrag{s03}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$z$\end{tabular}}%
\psfrag{s05}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$|\V{t}|_2$\end{tabular}}%
\psfrag{s06}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s07}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{0}%
\psfrag{x02}[t][t]{1}%
\psfrag{x03}[t][t]{2}%
\psfrag{x04}[t][t]{3}%
\psfrag{x05}[t][t]{4}%
\psfrag{x06}[t][t]{5}%
%
% yticklabels:
\psfrag{v01}[l][l]{0}%
\psfrag{v02}[l][l]{2}%
\psfrag{v03}[l][l]{4}%
\psfrag{v04}[l][l]{6}%
\psfrag{v05}[l][l]{8}%
\psfrag{v06}[l][l]{10}%
\psfrag{v07}[r][r]{-0.5}%
\psfrag{v08}[r][r]{0}%
\psfrag{v09}[r][r]{0.5}%
\psfrag{v10}[r][r]{1}%
\psfrag{v11}[r][r]{1.5}%
\psfrag{v12}[r][r]{2}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{2DTractionZ.matlab.eps}}%
\end{psfrags}%
%
% End 2DTractionZ.matlab.tex


==> Figures/L2Stress2.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}z\end{tabular}}%
\psfrag{s05}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\int_z^\infty g_z \rho dz$}%
\psfrag{s06}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\sigma_{zz}^0$}%
\psfrag{s07}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\sigma_{zz}$}%
\psfrag{s08}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\sigma_{zz}+\int_z^\infty t_z dz$}%
\psfrag{s09}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\int_z^\infty g_z \rho dz$}%
\psfrag{s11}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s12}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{-2}%
\psfrag{x02}[t][t]{0}%
\psfrag{x03}[t][t]{2}%
\psfrag{x04}[t][t]{4}%
\psfrag{x05}[t][t]{6}%
\psfrag{x06}[t][t]{8}%
\psfrag{x07}[t][t]{10}%
%
% yticklabels:
\psfrag{v01}[r][r]{0}%
\psfrag{v02}[r][r]{1}%
\psfrag{v03}[r][r]{2}%
\psfrag{v04}[r][r]{3}%
\psfrag{v05}[r][r]{4}%
\psfrag{v06}[r][r]{5}%
\psfrag{v07}[r][r]{6}%
\psfrag{v08}[r][r]{7}%
\psfrag{v09}[r][r]{8}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{L2Stress2.matlab.eps}}%
\end{psfrags}%
%
% End L2Stress2.matlab.tex


==> Figures/L2StressXX.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}z\end{tabular}}%
\psfrag{s05}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\sigma_{xx}`$}%
\psfrag{s06}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\sigma_{xx}^0$}%
\psfrag{s07}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\sigma_{xx}$}%
\psfrag{s08}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\sigma_{xx}`$}%
\psfrag{s10}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s11}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{-2}%
\psfrag{x02}[t][t]{0}%
\psfrag{x03}[t][t]{2}%
\psfrag{x04}[t][t]{4}%
\psfrag{x05}[t][t]{6}%
\psfrag{x06}[t][t]{8}%
\psfrag{x07}[t][t]{10}%
%
% yticklabels:
\psfrag{v01}[r][r]{0}%
\psfrag{v02}[r][r]{2}%
\psfrag{v03}[r][r]{4}%
\psfrag{v04}[r][r]{6}%
\psfrag{v05}[r][r]{8}%
\psfrag{v06}[r][r]{10}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{L2StressXX.matlab.eps}}%
\end{psfrags}%
%
% End L2StressXX.matlab.tex


==> Figures/L2Traction.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}z\end{tabular}}%
\psfrag{s05}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$g \rho$}%
\psfrag{s06}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$|\nabla\V{\sigma}_{zz}+\V{t}|$}%
\psfrag{s07}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$g \rho$}%
\psfrag{s09}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s10}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{-2}%
\psfrag{x02}[t][t]{0}%
\psfrag{x03}[t][t]{2}%
\psfrag{x04}[t][t]{4}%
\psfrag{x05}[t][t]{6}%
\psfrag{x06}[t][t]{8}%
\psfrag{x07}[t][t]{10}%
%
% yticklabels:
\psfrag{v01}[r][r]{0}%
\psfrag{v02}[r][r]{0.1}%
\psfrag{v03}[r][r]{0.2}%
\psfrag{v04}[r][r]{0.3}%
\psfrag{v05}[r][r]{0.4}%
\psfrag{v06}[r][r]{0.5}%
\psfrag{v07}[r][r]{0.6}%
\psfrag{v08}[r][r]{0.7}%
\psfrag{v09}[r][r]{0.8}%
\psfrag{v10}[r][r]{0.9}%
\psfrag{v11}[r][r]{1}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{L2Traction.matlab.eps}}%
\end{psfrags}%
%
% End L2Traction.matlab.tex


==> Figures/cg.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$x$\end{tabular}}%
\psfrag{s05}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\sigma$}%
\psfrag{s06}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\rho$}%
\psfrag{s07}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\sigma$}%
\psfrag{s09}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s10}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{-2}%
\psfrag{x02}[t][t]{-1.5}%
\psfrag{x03}[t][t]{-1}%
\psfrag{x04}[t][t]{-0.5}%
\psfrag{x05}[t][t]{0}%
\psfrag{x06}[t][t]{0.5}%
\psfrag{x07}[t][t]{1}%
\psfrag{x08}[t][t]{1.5}%
\psfrag{x09}[t][t]{2}%
\psfrag{x10}[t][t]{2.5}%
\psfrag{x11}[t][t]{3}%
%
% yticklabels:
\psfrag{v01}[r][r]{0}%
\psfrag{v02}[r][r]{1}%
\psfrag{v03}[r][r]{2}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{cg.matlab.eps}}%
\end{psfrags}%
%
% End cg.matlab.tex


==> Figures/cg2.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$x$\end{tabular}}%
\psfrag{s05}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\sigma_{base}$}%
\psfrag{s06}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\rho_{base}$}%
\psfrag{s07}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\sigma_{base}$}%
\psfrag{s09}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s10}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{-2}%
\psfrag{x02}[t][t]{-1.5}%
\psfrag{x03}[t][t]{-1}%
\psfrag{x04}[t][t]{-0.5}%
\psfrag{x05}[t][t]{0}%
\psfrag{x06}[t][t]{0.5}%
\psfrag{x07}[t][t]{1}%
\psfrag{x08}[t][t]{1.5}%
\psfrag{x09}[t][t]{2}%
\psfrag{x10}[t][t]{2.5}%
\psfrag{x11}[t][t]{3}%
%
% yticklabels:
\psfrag{v01}[r][r]{0}%
\psfrag{v02}[r][r]{1}%
\psfrag{v03}[r][r]{2}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{cg2.matlab.eps}}%
\end{psfrags}%
%
% End cg2.matlab.tex


==> Figures/static2d.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s02}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$x$\end{tabular}}%
\psfrag{s03}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$z$\end{tabular}}%
\psfrag{s05}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$|\V{t}|$\end{tabular}}%
\psfrag{s06}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s07}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s09}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$x$\end{tabular}}%
\psfrag{s10}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$z$\end{tabular}}%
\psfrag{s12}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$tr(\sigma)$\end{tabular}}%
\psfrag{s13}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s14}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{0}%
\psfrag{x02}[t][t]{0.5}%
\psfrag{x03}[t][t]{1}%
\psfrag{x04}[t][t]{0}%
\psfrag{x05}[t][t]{1}%
\psfrag{x06}[t][t]{2}%
\psfrag{x07}[t][t]{3}%
\psfrag{x08}[t][t]{4}%
\psfrag{x09}[t][t]{5}%
\psfrag{x10}[t][t]{0}%
\psfrag{x11}[t][t]{0.5}%
\psfrag{x12}[t][t]{1}%
\psfrag{x13}[t][t]{0}%
\psfrag{x14}[t][t]{1}%
\psfrag{x15}[t][t]{2}%
\psfrag{x16}[t][t]{3}%
\psfrag{x17}[t][t]{4}%
\psfrag{x18}[t][t]{5}%
%
% yticklabels:
\psfrag{v01}[l][l]{0}%
\psfrag{v02}[l][l]{0.1}%
\psfrag{v03}[l][l]{0.2}%
\psfrag{v04}[l][l]{0.3}%
\psfrag{v05}[l][l]{0.4}%
\psfrag{v06}[r][r]{-0.5}%
\psfrag{v07}[r][r]{0}%
\psfrag{v08}[r][r]{0.5}%
\psfrag{v09}[r][r]{1}%
\psfrag{v10}[r][r]{1.5}%
\psfrag{v11}[r][r]{2}%
\psfrag{v12}[l][l]{1}%
\psfrag{v13}[l][l]{2}%
\psfrag{v14}[l][l]{3}%
\psfrag{v15}[l][l]{4}%
\psfrag{v16}[l][l]{5}%
\psfrag{v17}[l][l]{6}%
\psfrag{v18}[r][r]{-0.5}%
\psfrag{v19}[r][r]{0}%
\psfrag{v20}[r][r]{0.5}%
\psfrag{v21}[r][r]{1}%
\psfrag{v22}[r][r]{1.5}%
\psfrag{v23}[r][r]{2}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{static2d.matlab.eps}}%
\end{psfrags}%
%
% End static2d.matlab.tex


==> Figures/t_dependence_momeq.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s05}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\Delta t=200$}%
\psfrag{s06}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\Delta t=1$}%
\psfrag{s07}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\Delta t=5$}%
\psfrag{s08}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\Delta t=10$}%
\psfrag{s09}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\Delta t=50$}%
\psfrag{s10}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\Delta t=100$}%
\psfrag{s11}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\Delta t=200$}%
\psfrag{s13}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s14}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{0}%
\psfrag{x02}[t][t]{5}%
\psfrag{x03}[t][t]{10}%
\psfrag{x04}[t][t]{15}%
\psfrag{x05}[t][t]{20}%
\psfrag{x06}[t][t]{25}%
\psfrag{x07}[t][t]{30}%
%
% yticklabels:
\psfrag{v01}[r][r]{-0.2}%
\psfrag{v02}[r][r]{-0.1}%
\psfrag{v03}[r][r]{0}%
\psfrag{v04}[r][r]{0.1}%
\psfrag{v05}[r][r]{0.2}%
\psfrag{v06}[r][r]{0.3}%
\psfrag{v07}[r][r]{0.4}%
\psfrag{v08}[r][r]{0.5}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{t_dependence_momeq.matlab.eps}}%
\end{psfrags}%
%
% End t_dependence_momeq.matlab.tex


==> Figures/t_dependence_momeq2.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{l}1\end{tabular}}%
\psfrag{s02}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{l}1\end{tabular}}%
\psfrag{s03}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$T$\end{tabular}}%
\psfrag{s04}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$||\vec{r}(z)|_2|_{L_2(\mathbb{R})}$\end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{$10^{0}$}%
\psfrag{x02}[t][t]{$10^{1}$}%
\psfrag{x03}[t][t]{$10^{2}$}%
%
% yticklabels:
\psfrag{v01}[r][r]{$10^{-2}$}%
\psfrag{v02}[r][r]{$10^{-1}$}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{t_dependence_momeq2.matlab.eps}}%
\end{psfrags}%
%
% End t_dependence_momeq2.matlab.tex


==> Figures/t_dependence_nu.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$z$\end{tabular}}%
\psfrag{s02}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\nu$\end{tabular}}%
\psfrag{s05}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\Delta t=200$}%
\psfrag{s06}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\Delta t=10$}%
\psfrag{s07}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\Delta t=50$}%
\psfrag{s08}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\Delta t=100$}%
\psfrag{s09}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$\Delta t=200$}%
\psfrag{s11}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s12}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{0}%
\psfrag{x02}[t][t]{5}%
\psfrag{x03}[t][t]{10}%
\psfrag{x04}[t][t]{15}%
\psfrag{x05}[t][t]{20}%
\psfrag{x06}[t][t]{25}%
\psfrag{x07}[t][t]{30}%
%
% yticklabels:
\psfrag{v01}[r][r]{0.4}%
\psfrag{v02}[r][r]{0.45}%
\psfrag{v03}[r][r]{0.5}%
\psfrag{v04}[r][r]{0.55}%
\psfrag{v05}[r][r]{0.6}%
\psfrag{v06}[r][r]{0.65}%
\psfrag{v07}[r][r]{0.7}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{t_dependence_nu.matlab.eps}}%
\end{psfrags}%
%
% End t_dependence_nu.matlab.tex


==> Figures/w_dependence_nu.matlab.tex <==
% generated by laprint.m
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s01}[t][t]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$z$\end{tabular}}%
\psfrag{s02}[b][b]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$\nu$\end{tabular}}%
\psfrag{s05}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$w=1$}%
\psfrag{s06}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$w=0.05$}%
\psfrag{s07}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$w=0.1$}%
\psfrag{s08}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$w=0.25$}%
\psfrag{s09}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$w=0.5$}%
\psfrag{s10}[l][l]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}$w=1$}%
\psfrag{s12}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
\psfrag{s13}[][]{\fontsize{10}{15}\fontseries{m}\mathversion{normal}\fontshape{n}\selectfont \color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c} \end{tabular}}%
%
% axes font properties:
\fontsize{10}{15}\fontseries{m}\mathversion{normal}%
\fontshape{n}\selectfont%
%
% xticklabels:
\psfrag{x01}[t][t]{0}%
\psfrag{x02}[t][t]{5}%
\psfrag{x03}[t][t]{10}%
\psfrag{x04}[t][t]{15}%
\psfrag{x05}[t][t]{20}%
\psfrag{x06}[t][t]{25}%
\psfrag{x07}[t][t]{30}%
%
% yticklabels:
\psfrag{v01}[r][r]{0.4}%
\psfrag{v02}[r][r]{0.45}%
\psfrag{v03}[r][r]{0.5}%
\psfrag{v04}[r][r]{0.55}%
\psfrag{v05}[r][r]{0.6}%
\psfrag{v06}[r][r]{0.65}%
\psfrag{v07}[r][r]{0.7}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{w_dependence_nu.matlab.eps}}%
\end{psfrags}%
%
% End w_dependence_nu.matlab.tex

